Boosting gets full Attention for Relational Learning

More often than not in benchmark supervised ML, tabular data is flat, i.e. consists of a single $m \times d$ (rows, columns) file, but cases abound in the real world where observations are described by a set of tables with structural relationships. Neural nets-based deep models are a classical fit to incorporate general topological dependence among description features (pixels, words, etc.), but their suboptimality to tree-based models on tabular data is still well documented. In this paper, we introduce an attention mechanism for structured data that blends well with tree-based models in the training context of (gradient) boosting. Each aggregated model is a tree whose training involves two steps: first, simple tabular models are learned descending tables in a top-down fashion with boosting's class residuals on tables' features. Second, what has been learned progresses back bottom-up via attention and aggregation mechanisms, progressively crafting new features that complete at the end the set of observation features over which a single tree is learned, boosting's iteration clock is incremented and new class residuals are computed. Experiments on simulated and real-world domains display the competitiveness of our method against a state of the art containing both tree-based and neural nets-based models.

==> remarks.tex <==
\newcommand{\noteRN}[1]{{\bf\color{red}RN -- #1}}

\section{\noteRN{Remarks}}

\eqref{eq:upattention} looks like a mechanism to make boosting more efficient (not necessarily to improve the rate) -- in theory, boosting could use all "downwards" features but it would be suboptimal. Here, aggregation "surfaces" the best choices of features downwards.

\eqref{eq:upaggregation} looks very much like an embryo of deep learning with a topology given by the tables' relationships (say "Relational topology", "Tables topology" ?). Why not replacing $\varphi$ by a classical NN activation function whose parameters would be learned ? (ReLU, pooling, etc.)



